MonoNeRD: NeRF-like Representations for Monocular 3D Object Detection

In the field of monocular 3D detection, it is common practice to utilize scene geometric clues to enhance the detector's performance. However, many existing works adopt these clues explicitly such as estimating a depth map and back-projecting it into 3D space. This explicit methodology induces sparsity in 3D representations due to the increased dimensionality from 2D to 3D, and leads to substantial information loss, especially for distant and occluded objects. To alleviate this issue, we propose MonoNeRD, a novel detection framework that can infer dense 3D geometry and occupancy. Specifically, we model scenes with Signed Distance Functions (SDF), facilitating the production of dense 3D representations. We treat these representations as Neural Radiance Fields (NeRF) and then employ volume rendering to recover RGB images and depth maps. To the best of our knowledge, this work is the first to introduce volume rendering for M3D, and demonstrates the potential of implicit reconstruction for image-based 3D perception. Extensive experiments conducted on the KITTI-3D benchmark and Waymo Open Dataset demonstrate the effectiveness of MonoNeRD. Codes are available at https://github.com/cskkxjk/MonoNeRD.

==> figs/bev-vis.tex <==
\begin{figure*}[t]
\begin{center}
    % \begin{tabular}%{\linewidth}
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
        % \centering
        \includegraphics[width=0.73\linewidth]{figs/left-rgb.png}
        % \caption{Input monocular image.}\label{fig:6(a)}
    \end{center}
    % \begin{tabular}%{\linewidth}
    \begin{center}
        % \centering
        \includegraphics[height=28mm]{figs/density_bar.png}
        \includegraphics[height=28mm]{figs/left-rgb/bev.png}
        \includegraphics[height=28mm]{figs/left-d/bev.png}
        \includegraphics[height=28mm]{figs/left-rgb-right-rgb/bev.png}
        \includegraphics[height=28mm]{figs/left-rgbd/bev.png}
        \includegraphics[height=28mm]{figs/left-rgbd-sdf/bev.png}
        \label{fig:short-b}
        % \caption{From left to right: visualizations for Experiment setting (c, d, g, e, f).}\label{fig:6(b)}
    % \end{tabular}
\end{center}
\caption{Visualizations of density features in bird's-eye-view (BEV), density is accumulated along with the height axis. (See Section \ref{sss:visualization}). From left to right: Experiment setting (c, d, g, e, f). Low density means the 3D space is empty, while high density means it is occupied. Zoom in for better details.}
\label{fig:visualization}
\end{figure*}

==> tables/ablation_2d_3d.tex <==
\begin{table}[h]
\begin{center}
\footnotesize
  \resizebox{0.48\textwidth}{!}{
  \begin{tabular}{l|ccc|ccc}
    \hline
    \multirow{2}*{Exp.}&\multicolumn{3}{c|}{Setting}&\multicolumn{3}{c}{$AP_{BEV}/AP_{3D}$}\\
    {} & $L_{rgb}^{left}$ + $L_{rgb}^{right}$ & $L_{depth}$ & $L_{sdf}$ & Easy & Moderate & Hard\\
    \hline
    1  &\checkmark &  &  & 25.49 / 18.20 & 19.56 / 14.11 &17.18 / 12.22\\
    2  & &\checkmark & & 26.91 / 18.72 & 20.87 / 14.54 & 18.57 / 12.60\\
    3  &\checkmark &\checkmark & & 27.60 / 20.07 & 20.61 / 14.66 &17.95 / 12.45\\
    4  & &\checkmark  &\checkmark &27.94 / 20.28 & 21.44 / \textbf{15.32} &18.82 / 13.48\\
    5  &\checkmark &\checkmark &\checkmark &\textbf{29.65 / 20.82} & \textbf{22.10} / 15.29 &\textbf{20.02 / 13.55}\\
    \hline
  \end{tabular}
}
\end{center}
\caption{Ablation of 2D and 3D supervisions. 
``$L_{rgb}^{left}+L_{rgb}^{right}$'': using stereo images (left and right RGB images) as implicit depth supervision (See Figure 5 in the main text), depth supervision exists implicitly under this setting; 
``$L_{depth}$'': using LiDAR depth labels as depth supervision; 
``$L_{sdf}$'': using SDF loss for explicit 3D supervision.
We can see that even explicit depth supervision is unavailable, our method still can learn depth information from stereo images.
}
\label{tab:2d-3d-supervisions}
\end{table}

==> tables/ablation_plane.tex <==
\begin{table}[h]
\begin{center}
  \scriptsize
  %\resizebox{0.45\textwidth}{!}{
   {
  \begin{tabular}{c|c|ccc}
    \hline
     \multirow{2}*{Exp.} &\multirow{2}*{D}&\multicolumn{3}{c}{$AP_{BEV}/AP_{3D}$}\\
    {} & {} & Easy & Moderate & Hard\\
    \hline
    a &36 & 26.54 / 17.50 & 20.16 / 13.84 & 18.23 / 12.02\\
    b &54 & 28.07 / 18.79 & 21.31 / 14.57 & 18.47 / 12.39\\
    c &72 & 29.03 / 20.64 & 22.03 / 15.44 & 19.41 / 13.99\\
    d &108 & 28.41 / 20.31 & 21.33 / 15.43 & 18.78 / 13.52\\
    \hline
  \end{tabular}
  }
\end{center}
\caption{Ablation of the number of sampled depth planes (``D'').}
\label{tab:sample-point}
\end{table}

==> tables/depth-vs-nerf.tex <==
\begin{table}[h]
\begin{center}
    \small
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{l|c|c|c}
    \hline
    %Module  & 2D backbone & The proposed module & Detection module\\
    ~ & CaDDN \cite{reading2021categorical} & Baseline & MonoNeRD \\
    \hline
    Model Size & 774M & 83M & 83M \\
    Backbone & ResNet-101 & ResNet-34 & ResNet-34 \\
    Depth Head & DeepLabV3 \cite{chen2017rethinking} & 2-Layer-CNN & None \\
    Depth Label & LiDAR/depth completion \cite{ku2018defense} & LiDAR & LiDAR \\
    3D Rep. & Depth-transformed & Depth-transformed & NeRF-like \\
    3D Det. Head & PointPillars \cite{lang2019pointpillars} & SECOND \cite{yan2018second} & SECOND \cite{yan2018second}\\
    LIGA-Auxilary & None & $L_{2d}, L_{im}$ & $L_{2d}, L_{im}$ \\
    \hline
    KITTI \textit{val} $AP_{3D}$ & 23.57/16.31/13.84 & 18.75/14.49/12.55 & 20.64/15.44/13.99\\
    KITTI \textit{test} $AP_{3D}$ & 19.17/13.41/11.46 & - & 22.75/17.13/15.63\\
    \hline
    \end{tabular}
    }
\end{center}
\caption{Comparison between CaDDN and MonoNeRD. We create a baseline for convenience and fair comparison. ``3D Rep.'' and ``3D Det. Head'' refer to 3D Representation and 3D Detection Head. Baseline = MonoNeRD - NeRF-like + CaDDN-transformation.}
\label{tab:depth-vs-nerf}
\end{table}

==> tables/generalization-gap.tex <==
% \begin{table}[h]
% \begin{center}
%   % \scriptsize
%   \resizebox{1.0\columnwidth}{!}{
%   \begin{tabular}{l|c|c|c}
%     \hline
%     ~ & KITTI \textit{val} & KITTI \textit{test} & Waymo \textif{val}\\
%     \hline
%     Train size & 3k & 7k & 50k \\
%     Test size & 3k & 7k & 40k \\
%     Category &\textit{Car} & \textit{Car} & \textit{Vehicle} \\
%     Metric & $AP_{3D|Iou=0.7}$ & $AP_{3D|Iou=0.7}$ &$mAP_{3D|Iou=0.5}^{overall}$\\
%     \hline
%     CaDDN \cite{reading2021categorical} & & & \\
%     DID-M3D \cite{peng2022did} & & & \\
%     MonoNeRD (ours) & & & \\
%     \hline
%     \textit{vs.} CaDDN & & &\\
%     \textot{vs.} DID-M3D & & &\\
%     \hline
%   \end{tabular}
%   }
% \end{center}
% \caption{Performance Gap with different data sizes.}
% \label{tab:generl-gap}
% \end{table}

\begin{table}[h]
\begin{center}
    \small
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{l|c|c|c}
    \hline
    %Module  & 2D backbone & The proposed module & Detection module\\
    ~ & KITTI \textit{val} & KITTI \textit{test} & Waymo \textit{val} \\
    \hline
    Train size & 3k & 7k & 50k \\
    Test size & 3k & 7k & 40k \\
    Class & Car & Car & Vehicle\\
    Metric & $AP_{3D}$ & $AP_{3D}$ & 3D mAP\\
    IoU & 0.7 & 0.7 & 0.5 \\
    Setting & Moderate & Moderate & Level 1/ Overall\\
    \hline
    CaDDN \cite{reading2021categorical} & 16.31 & 13.41 & 17.54 \\
    DID-M3D \cite{peng2022did} & 16.12 & 16.29 & 20.66 \\
    \hline
    MonoNeRD & 15.44 & 17.13 & 31.18\\
    \textit{vs.} CaDDN & -5.33\% & +27.74\% & +77.77\% \\
    \textit{vs.} DID-M3D & -4.22\% & +5.16\% & +50.92\% \\
    \hline
    \end{tabular}
    }
\end{center}
\caption{Performance gap with different data sizes.}
\label{tab:generl-gap}
\end{table}

==> tables/kitti_test_other.tex <==
\begin{table*}[ht]
\begin{center}
    \footnotesize
    \begin{tabular}{l|ccc|ccc}
    \hline
    \multirow{2}*{Methods}  & \multicolumn{3}{c|}{$Pedestrian \quad AP_{BEV}/AP_{3D}$}  & \multicolumn{3}{c}{$Cyclist \quad AP_{BEV}/AP_{3D}$}\\
    {}                    &Easy   &Moderate &Hard    &Easy  &Moderate  &Hard\\
    \hline
    M3D-RPN\cite{brazil2019m3d}  &5.65 / 4.92   &4.05 / 3.48   &3.29 / 2.94   &1.25 / 0.94   &0.81 / 0.65   &0.78 / 0.47\\
    D4LCN\cite{ding2020learning}  &5.06 / 4.55   &3.86 / 3.42   &3.59 / 2.83   &2.72 / 2.45   &1.82 / 1.67   &1.79 / 1.36\\
    MonoPair\cite{chen2020monopair} &10.99 / 10.02   &7.04 / 6.68   &6.29 / 5.53   &4.76 / 3.79   & 2.87 / 2.12   & 2.42 / 1.83\\
    MonoFlex\cite{zhang2021objects}  &10.36 / 9.43 &7.36 / 6.31 &6.29 / 5.26 &4.41 / 4.17 &2.67 / 2.35 &2.50 / 2.04\\
    CaDDN\cite{reading2021categorical} &14.72 / 12.87 &9.41 / 8.14 &8.17 / 6.76 &\textbf{9.67} / \textbf{7.00} &\textbf{5.38} / \textbf{3.41} &\textbf{4.75} / \textbf{3.30}\\
    LPCG\cite{peng2022lidar} &12.11 / 10.82 &7.92 / 7.33 &6.61 / 6.18 &8.14 / 6.98 &4.90 / 4.38 &3.86 / 3.56\\
    \hline
    MonoNeRD(ours) & \textbf{15.27}/ \textbf{13.20} &\textbf{9.66} / \textbf{8.26} & \textbf{8.28} / \textbf{7.02} & 5.24 / 4.73 & 2.80 / 2.48 & 2.55 / 2.16\\
    \hline
    \end{tabular}
\end{center}
\caption{Performance for \emph{Pedestrian} and \emph{Cyclist} on KITTI \emph{test}. The best results are \textbf{bold}.}
\vspace{-1mm}
\label{tab:ped-cyc}
\end{table*}

==> tables/latency.tex <==
\begin{table}[h]
\begin{center}
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{l|c|c|c}
    \hline
    %Module  & 2D backbone & The proposed module & Detection module\\
    ~  & 2D backbone & Our module & Detection module\\
    \hline
    Latency & 25.7ms & 91.5ms & 94.6ms \\
    Ratio & 12.13\% & 43.20\% & 44.66\%\\ 
    \hline
    \end{tabular}
    }
\end{center}
\vspace{-2mm}
\caption{Latency for different modules.}
\vspace{-3mm}
\label{tab:latency}
\end{table}

==> tables/vis-kitti-raw.tex <==
\begin{table}[h]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c|c|c}
\toprule
Video tag  & Raw data sequence & Index \\
\midrule
0 & {2011\_09\_26\_drive\_0005\_sync} & 0000000020-0000000090 \\
1 & {2011\_10\_03\_drive\_0042\_sync} & 0000000180-0000000210 \\
\bottomrule
\end{tabular} 
}
\vspace{-3mm}
\caption{Our selections for 3D occupancy visualization.}
\label{tab:kitti-raw}
\vspace{-4mm}
\end{table}

==> tables/waymo-all.tex <==
\begin{table*}[ht]
\begin{center}
    \footnotesize
    \begin{tabular}{l|cccc|cccc}
    \hline
    \multirow{2}*{Methods} & \multicolumn{4}{c|}{3D mAP / mAPH (IoU = 0.7)} & \multicolumn{4}{c}{3D mAP / mAPH (IoU = 0.5)}\\
    {} & Overall &0 - 30m & 30 - 50m & 50m - $\infty$ &Overall &0 - 30m & 30 - 50m & 50m - $\infty$\\
    \hline
    \multicolumn{9}{c}{LEVEL 1}\\
    \hline
    PatchNet (ECCV20)\cite{ma2020rethinking}  &0.39 / 0.37   &1.67 / 1.63   &0.13 / 0.12   &0.03 / 0.03   &2.92 / 2.74   &10.03 / 9.75  &1.09 / 0.96   &0.23 / 0.18\\
    CaDDN (CVPR21)\cite{reading2021categorical}  &\textbf{\textcolor{blue}{5.03 / 4.99}}   &\textbf{\textcolor{blue}{14.54 / 14.43}}   &\textbf{\textcolor{blue}{1.47 / 1.45}}   &\textbf{\textcolor{blue}{0.10 / 0.10}} &17.54 / 17.31   &\textbf{\textcolor{blue}{45.00 / 44.46}}   &9.24 / 9.11   &0.64 / 0.62\\
    PCT (NeurIPS21)\cite{wang2021progressive} &0.89 / 0.88   &3.18 / 3.15   &0.27 / 0.27   &0.07 / 0.07   &4.20 / 4.15   &14.70 / 14.54   &1.78 / 1.75   &0.39 / 0.39\\
    MonoJSG (CVPR22)\cite{lian2022monojsg}  &0.97 / 0.95   &4.65 / 4.59   &0.55 / 0.53   &0.10 / 0.09   &5.65 / 5.47   &20.86 / 20.26   &3.91 / 3.79   &0.97 / 0.92\\
    DEVIANT (ECCV22)\cite{kumar2022deviant}  &2.69 / 2.67   &6.95 / 6.90   &0.99 / 0.98   &0.02 / 0.02   &10.98 / 10.89   &26.85 / 26.64   &5.13 / 5.08   &0.18 / 0.18\\
    DID-M3D (ECCV22)\cite{peng2022did} & - / -   & - / -   & - / -   & - / -   & \textbf{\textcolor{blue}{20.66 / 20.47}}   &40.92 / 40.60   &\textbf{\textcolor{blue}{15.63 / 15.48}}   &\textbf{\textcolor{blue}{5.35 / 5.24}}\\
    \hline
    MonoNeRD-avg & \textbf{\textcolor{red}{10.66 / 10.56}} &\textbf{\textcolor{red}{27.84 / 27.57}} & \textbf{\textcolor{red}{5.40 / 5.36}} & \textbf{\textcolor{red}{0.72 / 0.71}} & \textbf{\textcolor{red}{31.18 / 30.70}} &\textbf{\textcolor{red}{61.11 / 60.28}} & \textbf{\textcolor{red}{26.08 / 25.71}} &\textbf{\textcolor{red}{6.60 / 6.47}}\\
    \quad\quad\quad\quad\quad-seed 1 &10.56 / 10.46   &27.36 / 27.13   &5.38 / 5.34   &0.65 / 0.65   &31.33 / 30.84   &61.33 / 60.51   &26.21 / 25.84   &6.60 / 6.47\\
    \quad\quad\quad\quad\quad-seed 2 &10.69 / 10.59   &27.84 / 27.59   &5.31 / 5.27   &0.75 / 0.74   &31.15 / 30.69   &60.70 / 59.91   &26.05 / 25.71   &6.54 / 6.41\\
    \quad\quad\quad\quad\quad-seed 3 &10.74 / 10.62   &28.31 / 27.99   &5.51 / 5.46   &0.76 / 0.75   &31.07 / 30.57   &61.31 / 60.43   &25.97 / 25.59   &6.65 / 6.53\\
    \hline
    \multicolumn{9}{c}{LEVEL 2}\\
    \hline
    PatchNet (ECCV20)\cite{ma2020rethinking}  &0.38 / 0.36   &1.67 / 1.63   &0.13 / 0.11   &0.03 / 0.03   &2.42 / 2.28   &10.01 / 9.73  &1.07 / 0.94   &0.22 / 0.16\\
    CaDDN (CVPR21)\cite{reading2021categorical}  &\textbf{\textcolor{blue}{4.49 / 4.45}}   &\textbf{\textcolor{blue}{14.50 / 14.38}}   &\textbf{\textcolor{blue}{1.42 / 1.41}}   &\textbf{\textcolor{blue}{0.09 / 0.09}}   &16.51 / 16.28   &\textbf{\textcolor{blue}{44.87 / 44.33}}   &8.99 / 8.86   &0.58 / 0.55\\
    PCT (NeurIPS21)\cite{wang2021progressive} &0.66 / 0.66   &3.18 / 3.15   &0.27 / 0.26   &0.07 / 0.07   &4.03 / 3.99   &14.67 / 14.51   &1.74 / 1.71   &0.36 / 0.35\\
    MonoJSG (CVPR22)\cite{lian2022monojsg}  &0.91 / 0.89   &4.64 / 4.65   &0.55 / 0.53   &0.09 / 0.09   &5.34 / 5.17   &20.79 / 20.19   &3.79 / 3.67   &0.85 / 0.82\\
    DEVIANT (ECCV22)\cite{kumar2022deviant}  &2.52 / 2.50   &6.93 / 6.87   &0.95 / 0.94   &0.02 / 0.02   &10.29 / 10.20   &26.75 / 26.54   &4.95 / 4.90   &0.16 / 0.16\\
    DID-M3D (ECCV22)\cite{peng2022did} & - / -   & - / -   & - / -   & - / -   &\textbf{\textcolor{blue}{19.37 / 19.19}}   &40.77 / 40.46   &\textbf{\textcolor{blue}{15.18 / 15.04}}  &\textbf{\textcolor{blue}{4.69 / 4.59}}\\
    \midrule
    MonoNeRD-avg & \textbf{\textcolor{red}{10.03 / 9.93}} &\textbf{\textcolor{red}{27.75 / 27.48}} & \textbf{\textcolor{red}{5.25 / 5.21}} & \textbf{\textcolor{red}{0.60 / 0.59}} & \textbf{\textcolor{red}{29.29 / 28.84}} &\textbf{\textcolor{red}{60.91 / 60.08}} & \textbf{\textcolor{red}{25.36 / 25.00}} & \textbf{\textcolor{red}{5.77 / 5.66}}\\
    \quad\quad\quad\quad\quad-seed 1 &9.93 / 9.84   &27.28 / 27.04   &5.23 / 5.19   &0.54 / 0.53   &29.43 / 28.97   &61.14 / 60.32   &25.49 / 25.13   &5.77 / 5.66\\
    \quad\quad\quad\quad\quad-seed 2 &10.05 / 9.96   &27.75 / 27.50   &5.16 / 5.13   &0.62 / 0.61   &29.26 / 28.83   &60.49 / 59.70   &25.33 / 25.00   &5.72 / 5.61\\
    \quad\quad\quad\quad\quad-seed 3 &10.10 / 9.99   &28.22 / 27.90   &5.36 / 5.31   &0.63 / 0.62   &29.18 / 28.71   &61.10 / 60.22   &25.25 / 24.88   &5.82 / 5.71\\
    \hline
    \end{tabular}
    \end{center}
    % \vspace{-3mm}
    %\caption{Performance for \emph{Pedestrian} and \emph{Cyclist} on KITTI \emph{test} at IOU threshold 0.5. The best results are \textbf{bold}.}
    \caption{Results on Waymo \emph{val} set. We obtain the values of other methods from their respective papers. Our method performs the best.}
    % \vspace{-1mm}
    \label{tab:waymo-all}
\end{table*}

==> tables/waymo-reproducibility.tex <==
\begin{table*}[ht]
\begin{center}
    \footnotesize
    \begin{tabular}{l|c|cccc|cccc}
    \hline
    \multirow{2}*{Method} & \multirow{2}*{Run}& \multicolumn{4}{c|}{3D mAP / mAPH (IoU = 0.7)} & \multicolumn{4}{c}{3D mAP / mAPH (IoU = 0.5)}\\
    {} & {} & Overall &0 - 30m & 30 - 50m & 50m - $\infty$ &Overall &0 - 30m & 30 - 50m & 50m - $\infty$\\
    \hline
    \multirow{9}*{MonoNeRD} &\multicolumn{9}{c}{LEVEL 1}\\
    \cline{2-10}
    {} &1 &10.56 / 10.46   &27.36 / 27.13   &5.38 / 5.34   &0.65 / 0.65   &31.33 / 30.84   &61.33 / 60.51   &26.21 / 25.84   &6.60 / 6.47\\
    {} &2 &10.69 / 10.59   &27.84 / 27.59   &5.31 / 5.27   &0.75 / 0.74   &31.15 / 30.69   &60.70 / 59.91   &26.05 / 25.71   &6.54 / 6.41\\
    {} &3 &10.74 / 10.62   &28.31 / 27.99   &5.51 / 5.46   &0.76 / 0.75   &31.07 / 30.57   &61.31 / 60.43   &25.97 / 25.59   &6.65 / 6.53\\
    {} &Avg & \textbf{{10.66 / 10.56}} &\textbf{{27.84 / 27.57}} & \textbf{{5.40 / 5.36}} & \textbf{{0.72 / 0.71}} & \textbf{{31.18 / 30.70}} &\textbf{{61.11 / 60.28}} & \textbf{{26.08 / 25.71}} &\textbf{{6.60 / 6.47}}\\
    \cline{2-10}
    {} &\multicolumn{9}{c}{LEVEL 2}\\
    \cline{2-10}
    {} &1 &9.93 / 9.84   &27.28 / 27.04   &5.23 / 5.19   &0.54 / 0.53   &29.43 / 28.97   &61.14 / 60.32   &25.49 / 25.13   &5.77 / 5.66\\
    {} &2 &10.05 / 9.96   &27.75 / 27.50   &5.16 / 5.13   &0.62 / 0.61   &29.26 / 28.83   &60.49 / 59.70   &25.33 / 25.00   &5.72 / 5.61\\
    {} &3 &10.10 / 9.99   &28.22 / 27.90   &5.36 / 5.31   &0.63 / 0.62   &29.18 / 28.71   &61.10 / 60.22   &25.25 / 24.88   &5.82 / 5.71\\
    {} &Avg & \textbf{{10.03 / 9.93}} &\textbf{{27.75 / 27.48}} & \textbf{{5.25 / 5.21}} & \textbf{{0.60 / 0.59}} & \textbf{{29.29 / 28.84}} &\textbf{{60.91 / 60.08}} & \textbf{{25.36 / 25.00}} & \textbf{{5.77 / 5.66}}\\
    \hline
    \end{tabular}
    \end{center}
    % \vspace{-3mm}
    %\caption{Performance for \emph{Pedestrian} and \emph{Cyclist} on KITTI \emph{test} at IOU threshold 0.5. The best results are \textbf{bold}.}
    \caption{Three different runs on on Waymo \emph{val} set.}
    % \vspace{-1mm}
    \label{tab:waymo-rep}
\end{table*}
